Deep Medial Voxels: Learned Medial Axis Approximations for Anatomical Shape Modeling

Shape reconstruction from imaging volumes is a recurring need in medical image analysis. Common workflows start with a segmentation step, followed by careful post-processing and,finally, ad hoc meshing algorithms. As this sequence can be timeconsuming, neural networks are trained to reconstruct shapes through template deformation. These networks deliver state-ofthe-art results without manual intervention, but, so far, they have primarily been evaluated on anatomical shapes with little topological variety between individuals. In contrast, other works favor learning implicit shape models, which have multiple benefits for meshing and visualization. Our work follows this direction by introducing deep medial voxels, a semi-implicit representation that faithfully approximates the topological skeleton from imaging volumes and eventually leads to shape reconstruction via convolution surfaces. Our reconstruction technique shows potential for both visualization and computer simulations.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/

For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf.tex          - A bare bones starter file for IEEE conference papers.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl.tex          - A bare bones starter file for IEEE journal papers.

bare_jrnl_comsoc.tex   - A bare bones starter file for IEEE Communications
                         Society journal papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_jrnl_transmag.tex - A bare bones starter file for IEEE Transactions
                         on Magnetics journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for an IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf.tex, bare_conf_compsoc.tex, bare_jrnl.tex,
                   bare_jrnl_comsoc.tex, bare_jrnl_compsoc.tex,
                   bare_jrnl_transmag.tex
***************************************************************************


==> plot.tex <==



\pgfplotsset{compat=1.12}
\pgfplotstableread[col sep=comma]{dataPos.dat}\mydataPos
\begin{figure}

\begin{tikzpicture}
\begin{axis}[width=\linewidth, height=5cm,
  legend style={legend columns=-1},
  legend to name={thelegend},
  name={theaxis},
 % xlabel=Landmark,
  ylabel=Limits of agreement (mm),
  xtick=data,
  xticklabels from table={\mydataPos}{subject},
  xticklabel style={font=\tiny}, 
  nodes near coords,
  nodes near coords style={font=\tiny, color=black},
  ybar,
  ymin=0,ymax=30,
  ytick={0,5,10,15,20,25},
  yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
}]
\addplot [color=gray!50,fill] table [x expr=\coordindex, y={Landmark}] \mydataPos;
\legend{Landmark position}
\end{axis}
\node [below] at (theaxis.below south) {\ref{thelegend}};
\end{tikzpicture}
\caption{Limits of agreement of the interoperator variability for the placement of the clinical landmarks calculated according to Jones et al.~\cite{Jones_2011}. The bias is zero in all cases and therefore not shown. \emph{All} refers to the overall variability among landmarks and operators. Higher variabilities for PAr, DAr, PDe and, particularly, DDe were expected due to their rather ill-defined nature. }
\label{fig:landmark_pos}
\end{figure}


==> plot2.tex <==




\pgfplotsset{compat=1.12}
\pgfplotstableread[col sep=comma]{data.dat}\mydata

\begin{figure*}
\begin{tikzpicture}%[font=\sffamily\small]
\begin{axis}[width=\linewidth, height=5cm,
  legend style={legend columns=-1},
  legend to name={thelegend},
  name={theaxis},
  %xlabel=Landmark,
  ylabel=Limits of agreement {$\mathbf{\phi}$} (deg),
  label style={font=\large},
  xtick=data,
  xticklabels from table={\mydata}{subject},
  ybar,
  ymin=0,ymax=35,
  nodes near coords,
  nodes near coords style={font=\tiny, color=black},
  ytick={0,5,10,15,20,25,30,35},
  yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
}]
\addplot [color=cyan!50,fill, bar width=0.0122\linewidth] table [x expr=\coordindex, y={Phi}] \mydata;
\addplot [color=lightgray,fill, bar width=0.0122\linewidth] table [x expr=\coordindex, y={PhiCL}] \mydata;
\addplot [color=teal!50,fill, bar width=0.0122\linewidth] table [x expr=\coordindex, y={PhiCNN}] \mydata;
%\legend{$\phi$ (manual), $\phi$ (centerline), $\phi$ (CNN)}
\end{axis}
\node [below] at (theaxis.below south) {\ref{thelegend}};
\end{tikzpicture}
\begin{tikzpicture}
\begin{axis}[width=\linewidth, height=5cm,
  legend style={legend columns=-1},
  legend to name={thelegend},
  name={theaxis},
  xlabel=Landmark,
  ylabel=Limits of agreement $\mathbf{\theta}$ (deg),
  label style={font=\large},
  xtick=data,
  xticklabels from table={\mydata}{subject},
  ybar,
  ymin=0,ymax=25,
  nodes near coords,
  nodes near coords style={font=\tiny, color=black},
  %ytick={0,4,8,12,16,20},
  yticklabel style={
        /pgf/number format/fixed,
        /pgf/number format/precision=2
}]
\addplot [color=cyan!50,fill, bar width=0.0122\linewidth] table [x expr=\coordindex, y={Theta}] \mydata;
\addplot [color=lightgray,fill, bar width=0.0122\linewidth] table [x expr=\coordindex, y={ThetaCL}] \mydata;
\addplot [color=teal!60,fill, bar width=0.0122\linewidth] table [x expr=\coordindex, y={ThetaCNN}] \mydata;
\legend{manual, centerline, CNN}
\end{axis}
\node [below] at (theaxis.below south) {\ref{thelegend}};
\end{tikzpicture}

\caption{Limits of agreement (95\%) of the interoperator variability for the two angles $(\theta,\phi)$ according to Jones et al.~\cite{Jones_2011} (absolute values, lower values are better). For a better readability we do not report the bias: as expected, this is zero in all cases, given we measure the variability against the mean. \emph{All} refers to the overall variability among landmarks and operators. Lower limits of agreement correspond to a higher reproducibility of the results. Given the same landmark positionings, \emph{manual} corresponds to the double-oblique reformation, \emph{centerline} to the centerline-derived planes, and \emph{CNN} to the CNN-derived planes. For a better readability and space limitation, the CNN limits of agreement refer only to the approach without uncertainty quantification (NoUQ).}
\label{fig:angle_loa}
\end{figure*}
